Surprising Negative Results for Generative Adversarial Tree Search

While many recent advances in deep reinforcement learning (RL) rely on model-free methods, model-based approaches remain an alluring prospect for their potential to exploit unsupervised data to learn environment model. In this work, we provide an extensive study on the design of deep generative models for RL environments and propose a sample efficient and robust method to learn the model of Atari environments. We deploy this model and propose generative adversarial tree search (GATS) a deep RL algorithm that learns the environment model and implements Monte Carlo tree search (MCTS) on the learned model for planning. While MCTS on the learned model is computationally expensive, similar to AlphaGo, GATS follows depth limited MCTS. GATS employs deep Q network (DQN) and learns a Q-function to assign values to the leaves of the tree in MCTS. We theoretical analyze GATS vis-a-vis the bias-variance trade-off and show GATS is able to mitigate the worst-case error in the Q-estimate. While we were expecting GATS to enjoy a better sample complexity and faster converges to better policies, surprisingly, GATS fails to outperform DQN. We provide a study on which we show why depth limited MCTS fails to perform desirably.

==> sections/old-5-Experiment.tex <==
\section{Experiments}  
We extensively study the performance of \GATS on a Atari-like game \textit{Pong, Asterix, Breakout, Crazy Climber} and \textit{Free way} using OpenAI Gym~\citep{1606.01540}. The \DQN architecture and the game design choices are fully borrowed from~\cite{mnih2015human}. The architecture of \GDM, Fig.~\ref{fig:gdm_generator}, extends the proposed U-Net model for the generator inspired by the \textsc{pix2pix} network~\citep{isola2017image}. The \GDM receives a state, sequence of actions, and a Gaussian noise vector\footnote{We set the noise to zero for deterministic environments.} and outputs the next state.\footnote{See Apx for detailed explanation on architecture and optimization procedure.} The \RP is a simple model with 3 outputs, one for each possible clipped reward. We train \GDM and \RP using prioritized weighted mini-batches of size 128 (more weight on recent samples), and update the two networks every 16 decision steps  of \GATS (4 times less frequently than the $Q$ update). We deploy \GATS as bounded-depth MCTS on the learned model \footnote{Note that MCTS in a deterministic environment corresponds to lookahead tree search.} and use the learned $Q$ values at the leaves. %Each sample of mini-batch consists of a trajectory of length $H$ where \GDM generates the simulated future frames using its self generated frames.
\paragraph*{Bias-Variance of $Q_{\theta}$.}
To observe the existing bias and variance in $Q_{\theta}$, we run solely \DQN on the game Pong, for $20M$ time steps. Fig.~\ref{fig:pongQ} shows 4 consecutive frames where the agent receives a negative score and Table.~\ref{fig:pongQ} shows the estimated Q values by \DQN for these steps. As we observe in  Fig.~\ref{fig:pongQ} and Table.~\ref{fig:pongQ}, at the time step $t$, the estimated Q value of all the actions are almost the same. The agent takes the \textit{down} action and the environment goes to the next state $t+1$. The second row of Table.~\ref{fig:pongQ} expresses the Q value of the actions at this new state. Since this transition does not carry any reward and the discount factor is close to 1, ($\gamma=0.99$) we expect the max Q values at time step $t+1$ to be close the $Q$ values of action \textit{down}, but it is very different.
%
\begin{figure}[ht]
\hspace{0.5cm}
\vspace*{-0.0cm}
   \begin{minipage}{0.1\textwidth}
\includegraphics[width=1\textwidth]{Fig/PongQ/pong1.eps}
\centering
   \end{minipage}%\hfill 
\begin{minipage}{0.1\textwidth}
\includegraphics[width=1\textwidth]{Fig/PongQ/pong2.eps}
\centering
\end{minipage}%\hfill 
\begin{minipage}{0.1\textwidth}
\includegraphics[width=1\textwidth]{Fig/PongQ/pong3.eps}
\centering
\end{minipage}%\hfill 
\begin{minipage}{0.1\textwidth}
\includegraphics[width=1\textwidth]{Fig/PongQ/pong4.eps}
\centering
\end{minipage}\hfill
\hspace*{-2.5cm}
\begin{minipage}{0.1\textwidth}
  \centering
  \footnotesize
  \begin{tabular}{l|cccr|rr}
    \multicolumn{1}{c}{}&\multicolumn{3}{c}{Action space} \\
    \toprule
Steps&stay&up&down\\
\midrule
$t$& 4.3918 & 4.3220 & 4.3933\\
$t+1$& 2.7985 & 2.8371 &2.7921\\
$t+2$&2.8089 & 2.8382 &2.8137\\
$t+3$& 3.8725 &3.8795 & 3.8690\\
    \bottomrule
  \end{tabular}
\end{minipage}\hfill 
% \vspace*{-0.3cm}
\caption{The sequence of four consecutive decision states, and corresponding learned Q function by \DQN at $t,t+1,t+2,t+3$ from left to right, where the agent loses the point.}
   \label{fig:pongQ}
%    \vspace*{-0.4cm}
\end{figure}
Moreover, in Fig.~\ref{fig:pong-bias} and Table.~\ref{fig:pong-bias} we investigate the case that the agent catches the ball. The ball is going to the right and agent needs to catch it. At time step $t$, the paddle is not on the direction of ball velocity, and as shown in Table.~\ref{fig:pong-bias}, the optimal action is \textit{down}. But a closer look at the estimated Q value of action \textit{up} reveals that the Q value for both action \textit{up} is unreasonably close, when it could lead to losing the point.
%
\begin{figure}[ht]
\hspace{1.5cm}
\vspace*{-0.2cm}
\centering
   \begin{minipage}{0.1\textwidth}
\includegraphics[width=1\textwidth]{Fig/PongQ/pong5.eps}
\centering
 \end{minipage}
\begin{minipage}{0.1\textwidth}
\includegraphics[width=1\textwidth]{Fig/PongQ/pong6.eps}
\centering
\end{minipage}\hfill
% \vspace*{-0.4cm}
\hspace*{-1.cm}
\begin{minipage}{0.1\textwidth}
  \centering
  \footnotesize
  \begin{tabular}{l|cccr|rr}
    \multicolumn{1}{c}{}&\multicolumn{3}{c}{Action space} \\
    \toprule
Steps&stay&up&down\\
\midrule
$t$& 1.5546 & 4.5181&   4.5214\\
    \bottomrule
  \end{tabular}
\end{minipage}\hfill
\caption{States at $t-1\rightarrow t$ and the corresponding Q function learned through \DQN at time $t$.}
   \label{fig:pong-bias}
%    \vspace*{-0.4cm}
\end{figure}
Lastly, we studied the existing errors in the estimation of the $Q$ function using \DQN. In Table.\ref{fig:pongQ}, if the agent could roll-out even one step before making a decision, it could observe negative consequence of action \textit{down}. The positive effect of the roll-out is more significant in earlier stages of $Q$ learning, where the $Q$ estimation is more off.




We run \GATS with $1,2,3$, and $4$ steps lookahead ($GATS1,GATS2,GATS3,GATS4$) and show its performance improvement over \DQN in ~Fig.~\ref{fig:gatsperformance}~\textit{(left)}. 
~Fig.~\ref{fig:gatsperformance}~\textit{(right)} shows the \RP prediction accuracy. We observe that when the transition phase occurs at decision step $1$M, the \RP model mis-classifies the positive rewards. But the \RP rapidly adapts to this shift and reduces the classification error to less than 2 errors per episode.
%
As DRL methods are data hungry, we can re-use the data to efficiently learn the model dynamics. Fig.~\ref{fig:exp} shows how accurate the \GDM can generate next $9$ frames just conditioning on the first frame and the trajectory of actions. This trajectory is generated at decision step $100k$. Moreover, we extend our study to the case where we change the model dynamics by changing the game mode. In this case, by going from default mode to alternate mode in pong, the opponent paddle gets halved in size. We expected that in this case, where the game became easier, the \DDQN agent would preserve its performance but surprisingly it gave us the most negative score possible, i.e -21 and broke. Therefore, we start fine tuning \DDQN and took 3M time step (12M frame) to master the game again. It is worth noting that it takes \DDQN 5M time step (20M frame) to master from scratch. While \DDQN shows a vulnerable and undesirably breakable behaviour to this scenario, \GDM and \RP thanks to their detailed design, adapt to the new model dynamics in 3k samples, which is amazingly smaller (see detail in \ref{Domain Adaptation})
\input{GAN-fig}
%
%
\begin{figure}[ht]
\vspace*{-0.3cm}
   \begin{minipage}{1\textwidth}
   \centering
\includegraphics[width=0.4\linewidth]{Fig/GATS.eps}
%      \vspace*{-0.8cm}
%      \caption*{(a)}
\includegraphics[width=0.4\linewidth]{Fig/RewGATS.eps}
%
   \end{minipage} 
\vspace*{-0.2cm}
\caption{\textit{left}:\GATS learns a better policy faster than plain \DQN ($2$ times faster). \GATS$k$ denotes \GATS of depth $k$. \textit{right}: Accuracy of \RP. The $Y$ axis shows the number of mistakes per episode and each episode has average length of $2k$, so the acc is almost always around $99.8\%$. This accuracy is consistent among runs and different lookahead lengths.}

\label{fig:gatsperformance}
% \vspace*{-0.4cm}
\end{figure}
%
In addition to \GATS on \DQN, we also study two other set of experiments on \DDQN. Since Fig.~\ref{fig:gatsperformance} shows that the deeper roll-outs beyond one step do not provide much additional benefit for Pong, we focus on one-step roll-outs for the next two experiments. 
%
In the first experiment, we equip \GATS+\DDQN with the mentioned Wasserstein-optimism approach, and compare it with \DDQN and plain \GATS+\DDQN, which both use $\varepsilon$-greedy based approaches for exploration. In Fig.~\ref{fig:ddqn}\textit{left},~ we observe that this optimism heuristic is helpful for better exploration.
%

In the second experiment, we investigate the effect of prioritizing training samples for the \GDM, fresher samples are more probable to be chosen, which we do in all experiments reported in Fig.~\ref{fig:ddqn}\textit{left}. We study the case where the input samples to \GDM are instead chosen uniformly at random from the replay buffer in  Fig.~\ref{fig:ddqn}\text{right}. In this case the \GATS learns a better policy faster at the beginning of the game, but the performance stays behind \DDQN, due to the shift in the state distribution. It is worth mentioning that for optimism based exploration, there is no $\varepsilon$-greedy, which is why it gets close to the maximum score of $21$. We tested \DDQN and \GATS-\DDQN with $\varepsilon=0$, and they also perform close to $21$. We further extend the study of \GDM to more games \ref{fig:gdm_rollouts} and observed same robust behaviour as Pong. We also tried to apply \GATS to more games, but were not able to extend it due to mainly its high computation cost. We tried different strategies of storing samples generated by MCTS, e.g. random generated experience, trajectory followed by Q on the tree, storing just leaf nodes, max leaf, also variety of different distributions, e.g. geometric distributing, but again due the height cost of hyper parameter tuning we were not successful to come up with a setting that \GATS works for other games

\begin{figure}[ht]
\vspace*{-0.2cm}
   \begin{minipage}{1\textwidth}
   \centering
\includegraphics[width=0.4\linewidth]{Fig/optimism.eps}
%      \vspace*{-0.8cm}
%      \caption*{(a)}
\includegraphics[width=0.4\linewidth]{Fig/Pong_full_replay.eps}

   \end{minipage} 
\caption{\textit{left}:The optimism approach for \GATS improves the sample complexity and learns a better policy faster. \textit{right}: Sampling the replay buffer uniformly at random to train \GDM, makes \GDM slow to adapt to novel parts of state space.}
\label{fig:ddqn}
%    \vspace*{-0.4cm}
\end{figure}











==> sections/old-5-Experiment1.tex <==
\section{Experiments}  
We study the performance of \GATS on the game \textit{Pong} from Arcade Learning Environment (ALE)~\citep{bellemare2013arcade} through OpenAI Gym \citep{1606.01540}. Since in our \GATS implementation, we used \DQN as a learning block for Q-function, we study how much improvement \GATS can achieve by reduce the biases due to \DQN $Q$ estimation in the terms of sample complexity and final score. 

For the design choice of the game, each decision step corresponds to four frames of ALE, and each state of the environment is defined as four consecutive frames of decision steps in gray scale. 

\paragraph*{\DQN Architecture}
The \DQN architecture is borrowed from~\cite{mnih2015human}. The input is a $4\times 84\times 84$ tensor followed by three convolutional layers. The first layers consists of 32 filters of size 8, the second layer consists of 64 filters of size 4 and the third layer consists of 64 filters of size 3. The result-in output of these 3 convolutional layers is fed into two fully connected layers with hidden layer of size 512 and output layer of size as number of actions.

\paragraph*{\GDM Architecture}
The architecture of \GDM is inspired by \textsc{pix2pix} network~\citep{isola2017image}. We deploy the proposed U-Net model as the generator. It consists of five convolutional layers in order to construct the bottle neck where we concatenate it with the input action and followed with five de-convolutional layers to generate next frame. The discriminator  model has three convolutional layers where we concatenate the input action with the output of these layers which is followed with a fully connected layer. 

\paragraph*{\RP Architecture} The \RP is a simple model with 3 outputs. It consist of 3 convolutional layers, where, similar to the discriminator, we concatenate the input action with the output of these 3 layers which is also followed with a fully connected layer. 

We train \GDM using mini-batches of size 20 and update it every 10 decision steps of \GATS. Each sample of mini-batch consists of a trajectory of length $H+1$ where \GDM generates the simulated future frames using its self generated frames. We do the same number of updates for \RP. For \DQN part, we update it every 4 decision steps using mini-batch of size 32. 

\paragraph*{Bias-Variance of $Q_{\theta}$.}
To observe the effect of systematic and estimation biased of $Q_{\theta}$, in addition its estimation variance, we run solely \DQN on the game Pong, for $5M$ times steps, the time when the greedy policy almost reaches the maximum per episode possible return of $21$. We run the $\varepsilon$-greedy policy of learned Q-function in order to observe the different scenarios, otherwise, the model does not score negative. Fig.~\ref{fig:pongQ} express 4 consecutive frames at decision steps where the agent receive a negative score and Table.~\ref{table:Q-lose} shows the estimated Q values by \DQN for these steps. The action space of the game Pong consists of three actions, $\{stay, up, down\}$. As we observe in  Fig.~\ref{fig:pongQ} and Table.~\ref{table:Q-lose}, at the time step $t$, the estimated Q value of all the actions are almost the same. The agent makes \textit{down} decision and the environment goes to the next state. The second row of Table.~\ref{table:Q-lose}  expresses the Q value of the actions at this new state. Since this transition does not carry any reward and discount factor is close to 1, ($\gamma=0.99$) we expect the Q values at time step $t+1$ to be close the $Q$ values of action \textit{down} but they are very different. On the other hand it is acceptable that at time step $t+2$ the expected Q values are small, but since the agent receives its negative score at times step $t+3$ we do not expect that the estimated $Q$ at time step $t+3$ to be larger than time step $t+2$. 

\begin{figure}[ht]
\vspace*{-0.0cm}
   \begin{minipage}{0.1\textwidth}
\includegraphics[width=1.5\textwidth]{Fig/PongQ/pong1.png}
\centering
   \end{minipage}\hfill 
\begin{minipage}{0.1\textwidth}
\includegraphics[width=1.5\textwidth]{Fig/PongQ/pong2.png}
\centering
\end{minipage}\hfill 
\begin{minipage}{0.1\textwidth}
\includegraphics[width=1.5\textwidth]{Fig/PongQ/pong3.png}
\centering
\end{minipage}\hfill 
\begin{minipage}{0.1\textwidth}
\includegraphics[width=1.5\textwidth]{Fig/PongQ/pong4.png}
\centering
\end{minipage}\hfill 
\caption{The sequence of four consecutive decision states, $t,t+1,t+2,t+3$ from left to right, where the agent losses a point.}
   \label{fig:pongQ}
   \vspace*{-0.4cm}
\end{figure}

% \begin{table}[!ht]
% \begin{center}
% \hspace*{-0.2cm}
%  \begin{tabular}{|c|c |c|c|} 
%  \hline
%  Steps  & stay & up & down\\ [0.5ex] 
%  \hline
% $t$ & 4.39185286 & 4.32205486 & 4.39337826\\ [0.5ex] 
% $t+1$ & 2.79852176 & 2.83711505 &2.79211664 \\ [0.5ex] 
% $t+2$ & 2.80890489 & 2.838274 &2.81375718\\ [0.5ex] 
% $t+3$ & 3.8725996 &3.87951708 & 3.86904812\\ [0.5ex] 
% \hline
% \end{tabular}
% \end{center}
% \caption{The Q function learned by \DQN}
% \label{table:Q-lose}
% \vspace*{-0.4cm}
% \end{table}






\begin{table}[!ht]
  \centering
  \caption{
    The Q function, learned by \DQN, when the agent scores a negative point
  }
  \footnotesize
  \begin{tabular}{l|cccr|rr}
    \multicolumn{1}{c}{}&\multicolumn{3}{c}{Action space} \\
    \toprule
Steps&stay&up&down\\
\midrule
$t$& 4.3918 & 4.3220 & 4.3933\\
$t+1$& 2.7985 & 2.8371 &2.7921\\
$t+2$&2.8089 & 2.8382 &2.8137\\
$t+3$& 3.8725 &3.8795 & 3.8690\\
    \bottomrule
  \end{tabular}

  \label{table:Q-lose}
\end{table}



% \begin{table}[!t]
%   \centering
%   \caption{
%     The Q function learned by \DQN
%   }
%   \footnotesize
%   \begin{tabular}{lr|crrr|rr}
%     \multicolumn{2}{c}{} & \multicolumn{4}{c}{\emph{Identity Verification}} & \multicolumn{2}{c}{\emph{Sample Diversity}} \\
%     \toprule
% Dataset&Mem&Judge&AUC&Acc.&FAR&ID-Div&All-Div\\
% \midrule
% \emph{MS-Celeb-1M}&-&FN&$.913$&$.867$&$.045$&$.621$&$.699$\\
% AC-DCGAN&$131$~MB&FN&$.927$&$.851$&$\mathbf{.083}$&$.497$&$.666$\\
% SD-DCGAN&$57$~MB&FN&$.823$&$.749$&$.201$&$.521$&$.609$\\
% SD-DCGAN-SC&$\mathbf{47}$~MB&FN&$.831$&$.757$&$.180$&$.560$&$.637$\\
% SD-DCGAN $k4$&$75$~MB&FN&$.852$&$.776$&$.227$&$.523$&$.614$\\
% SD-DCGAN $d_I25$&$57$~MB&FN&$.835$&$.764$&$.222$&$.526$&$.615$\\
% SD-DCGAN $d_I75$&$57$~MB&FN&$.816$&$.743$&$.268$&$.517$&$.601$\\
% SD-BEGAN&$68$~MB&FN&$\mathbf{.928}$&$\mathbf{.857}$&$.110$&$\mathbf{.588}$&$\mathbf{.673}$\\
% \midrule
% \textdagger{}\emph{MS-Celeb-1M}&-&Us&-&$.850$&$.110$&$.621$&$.699$\\
% *\emph{MS-Celeb-1M}&-&MT&-&$.759$&$.035$&$.621$&$.699$\\
% *AC-DCGAN&$131$~MB&MT&-&$\mathbf{.765}$&$\mathbf{.090}$&$.497$&$.666$\\
% *SD-DCGAN $k4$&$75$~MB&MT&-&$.688$&$.147$&$.523$&$.614$\\
% *SD-BEGAN&$\mathbf{68}$~MB&MT&-&$.723$&.096&$\mathbf{.588}$&$\mathbf{.673}$\\
%     \bottomrule
%   \end{tabular}

%   \label{facepairs}
% \end{table}




Moreover, in Fig.~\ref{fig:pong-bias} and Table.~\ref{table:Q-bias} we investigate the case that the agent catches the ball. The ball is going to the right and agent needs to catch it. At times step $t$, the paddle is not in the direction of ball velocity and as it is shown in Table.~\ref{table:Q-bias}, the optimal action is going \textit{down}. But a closer look at the estimated Q value of action \textit{up} reveals that the Q value for both of this actions are unreasonably close and action \textit{up} might end up to losing the point.

\begin{figure}[ht]
\vspace*{-0.0cm}
   \begin{minipage}{0.15\textwidth}
\includegraphics[width=1.5\textwidth]{Fig/PongQ/pong5.png}
\centering
   \end{minipage}\hfill 
\begin{minipage}{0.15\textwidth}
\includegraphics[width=1.5\textwidth]{Fig/PongQ/pong6.png}
\centering
\end{minipage}\hfill 
\caption{The sequence of two consecutive decision states, $t-1,t$ from left to right, where the agent catch the ball.}
   \label{fig:pong-bias}
   \vspace*{-0.4cm}
\end{figure}

% \begin{table}[!ht]
% \begin{center}
% \hspace*{-0.2cm}
%  \begin{tabular}{|c|c |c|c|} 
%  \hline
%  Steps  & stay & up & down\\ [0.5ex] 
%  \hline
% $t$ & 1.55463457 & 4.51810169 &   4.52144527\\ [0.5ex]  
% \hline
% \end{tabular}
% \end{center}
% \caption{The Q function learned by \DQN}
% \label{table:Q-bias}
% \vspace*{-0.4cm}
% \end{table}


\begin{table}[!ht]
  \centering
  \caption{
    The Q function, learned by \DQN, when the agent catches the ball
  }
  \footnotesize
  \begin{tabular}{l|cccr|rr}
    \multicolumn{1}{c}{}&\multicolumn{3}{c}{Action space} \\
    \toprule
Steps&stay&up&down\\
\midrule
$t$& 1.5546 & 4.5181&   4.5214\\
    \bottomrule
  \end{tabular}

  \label{table:Q-bias}
\end{table}


\input{GAN-fig}

\paragraph*{\GATS on Pong, performance and sample complexity}
Lastly we studied the existing errors in the estimation of the Q function using \DQN. As, for example, it is expressed in Table.\ref{table:Q-lose}, if the agent could roll-out before making decision, even-if it is just one step look ahead) it could realize the negative return of making action down. The positive effect of the roll-out is more significant in earlier stage of learning Q where the estimation of Q is more off. This empirical study encourages using more to investigate \GATS. 

We run \GATS{}s with $1,2,3$, and $4$ steps lookahead $GATS1,GATS2,GATS3,GATS4$  for $5M$ time step and show its improvement over \DQN. Fig.~\ref{fig:gatsperformance} shows the significance of \GATS over \DQN. As argued before, even one step look head can provide a better estimate of Q value and therefore improves the sample complexity of the learning method by factor of two. 

Fig.~\ref{fig:RFperformance} shows the reward prediction accuracy of \RP. At the very beginning, when mostly the negative scores are observed, it learn how to predict them. Later when the transition phase occurs, the jump at time step $1M$ in Fig.~\ref{fig:gatsperformance}, the agent starts to catch the balls and score. This distribution shift causes the \RP model to miss-classification the positive rewards. But it rapidly adapts to this shift and reduces the classification error to less than 2 errors per episode.

As DRL methods are data hungry, we can re-use the data to learn the model dynamics. Fig.~\ref{fig:exp} shows how accurate the \GDM can generate the next $9$ frames, conditioning only on the first state and the trajectory of actions. This trajectory is generated at decision step $150k$.

\begin{figure}[ht]
\vspace*{-0.0cm}
   \begin{minipage}{1\textwidth}
\includegraphics[width=0.5\linewidth]{Fig/GATS.png}
%      \vspace*{-0.8cm}
%      \caption*{(a)}
   \end{minipage}  
\caption{\GATS learns a better policy faster than plain \DQN ($2$ times faster). \GATS{}k denotes \GATS of depth k. }
   \label{fig:gatsperformance}
   \vspace*{-0.4cm}
\end{figure}



\begin{figure}[ht]
\vspace*{-0.0cm}
   \begin{minipage}{1\textwidth}
\includegraphics[width=0.5\linewidth]{Fig/RewGATS.png}
%      \vspace*{-0.8cm}
%      \caption*{(a)}
   \end{minipage}  
\caption{Number of wrongly classified rewards per episode.
\RP predicts the reward with a significantly low error rate. When \GATS adaptively learns different policies and explore new parts of the state space, \RP immediately adjusts to the new distribution and predicts rewards with high accuracy}
 \label{fig:RFperformance}
   \vspace*{-0.4cm}
\end{figure}







==> sections/old3-1BiasVariance.tex <==
In the previous section, we discussed the \DQN objective function, Eq.~\ref{eq:reg}, 
which is an inherently biased estimator. 
In the next section, we demonstrate 
how big these biases can be in practice. %Moreover, in addition to \DQN and statistical biases, the learned Q can suffer from variance due to low samples regime in the sequential regressions defined in \DQN. 
Let $\wh{\cdot}$ denote an estimate for a given quantity 
and $e_Q$ be the upper bound on estimation error in $Q$ function (bias+variance);
$|Q(x,a)- \wh{Q}(x,a)|\leq e_Q~,~\forall x,a$. 
For any given rollout policy $\piroll$, 
using \GDM, \RP, and estimated Q, 
the expected return is given by the following expression:
%$\xi_p(\piroll,x)$
%(thesubscript $p$ stands for predicted)
\begin{align*}%\label{eq:offMCTS}
\!\!\xi_p(\piroll,x)\!:=\!\E_{\piroll,\GDM,\RP}\!\left[\!\left(\sum_{h=0}^{H-1}\!\!\gamma^h\wh{r}_h\!\!\right)\!\!+\!\gamma^H\!\max_a\wh{Q}({x}_H,a)\Big| x\right]
\end{align*}
% Since we use the generators to generate states (frames) the generated state $\wh x$ corresponding to its correspondence $x$ might graphically be a bit different from $x$ while here we considers  
% It is worth noting that we denote $\wh x$  as the generated states and reward while there is a mapping  
Since this expectation is estimated with
given \GDM ,\RP and the estimated $Q$-function, 
\GATS efficiently estimates this expected return 
without any interaction with the real environment. 
Let $\xi(\piroll,x)$ denote the same quantity 
under the ground truth model
\begin{align*}
\xi(\piroll,x) :=
\E_{\piroll}\left[\left(\sum_{h=0}^{H-1}\gamma^hr_h\right)+\gamma^H\max_a{Q}({x}_H,a)\Big| x\right]
\end{align*}
Moreover, for the \RP and \GDM, where $\wh{T}$ and $\wh{r}$ 
are the estimated transition kernel and reward function \footnote{In the latter sections, 
we study $e_R$ and $e_T$, Fig.~\ref{fig:exp}, observing
that they are surprisingly small in practice, 
e.g. \RP, on average, makes less than two mistakes per episode in Pong} we consider $\forall x,{x}',a\in\X,\A$ 
\begin{align*}
\sum_{a}\left|\Big(r(x,a)-\wh{r}({x},a)\Big)\right|\leq e_R,~~~~~~~~\sum_{x'}\left|\Big(T(x'|x,a)-\wh{T}({x}'|x,a)\Big)\right|&\leq e_T
\end{align*}

\begin{proposition}\label{thm:BV}[Model-based Model-free trade-off] 
If \GATS is run to estimate the $Q$ function 
using \DQN procedure with the estimated model of the environment, \GDM and \RP,  the deviation in estimating $\xi_p(\piroll,x)$ $\forall~x$ and $\piroll$ is bounded as;
\begin{align}
&\!\!\!\!\!|\xi_p(\piroll,x)-\xi(\piroll,x)|\!\!\leq \!\frac{1-\gamma^{H}+H\gamma^{H}(1-\gamma)}{(1-\gamma)^2}e_T+\frac{1-\gamma^{H}}{1-\gamma}e_R+\gamma^He_Q\!
\end{align}
Proof in the Appendix~\ref{sec:proof} 
\end{proposition}

%
%
Proposition.~\ref{thm:BV} provides an insight to the contribution of error terms in the \GATS expected return $\xi_p(\piroll,x)$.  The exponential vanishing error in $Q$ estimation comes at the cost of error in the model estimation. Therefore, the agent can choose $H$, the depth of roll-out, in such a way to minimize the estimation error through approximating the upper bound on error terms.
%
%
% \begin{align*}%\label{eq:qgan}
% \centering
% \left(Q(\wh{x}_{H},a_{t+H};\theta')-r_{t+H}-\gamma \max_{a'}Q(x_{t+H+1},a';\theta^{target})\right)^2
% \end{align*}
% and update $\theta'$ in order to minimize this loss.



==> sections/old3-Preliminaries.tex <==
Consider an MDP $M=\langle \X, \A, T, R,P_0,\gamma\rangle$, 
with state space $\X$, action space $\A$, 
initial state distribution $P_0$, transition kernel $T$, reward distribution $R$ with $[0,1]$-bounded mean, and discount factor $0\leq\gamma<1$. 
The agent's objective is to find a policy $\pi:=\X \rightarrow \A$
that maximizes the overall expected discounted reward 
%$\eta^*:=\eta(\pi^*) = \max_{\pi}\lim_{N\rightarrow\infty}\E_{\pi}\left[\sum_{t=0}^N \gamma^tr_t|x_0\sim P_0\right]$.
For a policy $\pi$, $Q_{\pi}(x,a)$ denotes the expected return of action $a$ at state $x$, then following policy $\pi$. %:=\lim_{N\rightarrow\infty}\E_{\pi}\left[\sum_{t=0}^N \gamma^tr_t|x_0 = x,a_0=a\right]$. 
Following Bellman equation, we can learn the Q function by minimizing the following loss over samples:
\begin{align}\label{eq:double}
\left(Q(x,a)-\E_{\pi}\left[r+\gamma Q(x',a')\right|x,a]\right)^2
\end{align}
Since in RL we do not have access internal expectation, we instead minimize the Bellman residual~\citep{schweitzer1985generalized}\citep{lagoudakis2003least,antos2008learning} which has been extensively used in DRL literature~\citep{mnih2015human,van2016deep}: 
\begin{align*}
\!\!\!\E_{\pi}\!\!\left[\!\left(Q(x,a)\!-\!\left(r+\gamma Q(x',a')\right)\right)^2\!\Big|x,a\right]\!\!
=\!\!\left(\!Q(x,a)\!-\!\E_{\pi}\!\!\left[r\!+\!\gamma Q(x'\!,\!a')\Big|x,a\right]\!\right)^2\!\!\!\!+\!\!\textnormal{Var}_\pi\!\!\left(\!r\!+\!\gamma Q(x',a')\Big|x,a\!\right)
\end{align*}
% \begin{align*}
% &\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\E_{\pi}\left[\left(Q(x,a)-\left(r+\gamma Q(x',a')\right)\right)^2\!\Big|xa\right]\\
% &=\left(Q(x,a)-\E_{\pi}\left[r+\gamma Q(x',a')\Big|x,a\right]\!\right)^2+\textnormal{Var}_\pi\left(r+\gamma Q(x',a')\Big|x,a\right)
% \end{align*}
% \begin{align*}
% &\E_{\pi}\left[\left(Q(x,a)-\left(r+\gamma Q(x',a')\right)\right)^2\!\Big|x,a\right]\\
% &\quad\quad\quad\quad=\left(Q(x,a)-\E_{\pi}\left[r+\gamma Q(x',a')\Big|x,a\right]\!\right)^2+\textnormal{Var}_\pi\left(r+\gamma Q(x',a')\Big|x,a\right)
% \end{align*}
%
The Bellman residual is the sum Eq.~\ref{eq:double} 
and an additional variance term, rustling in a biased estimation of Q function. \DQN deploys target network in order to mitigate this bias and minimizes:
%
\begin{align}\label{eq:reg}
\hspace*{-0.3cm}\L(Q,Q^{\text{target}}) \!=\! \E_{\pi}\!\left[\left(Q(x,a)\!-r\!-\!\gamma Q^{target}(x',a')\right)^2\right]\!\!\!\!
\end{align}
In addition to this bias, 
there are statistical biases
due to limited capacity of network, 
optimization algorithm, 
model mismatch, 
as well as bias induced by the max operator or choice of $a'$~\citep{thrun1993issues}. 
In the next section, 
we theoretically and empirically 
study the effect of these biases and show how \GATS addresses these undesirable effects.
%
% \paragraph{Wasserstein metric adversarial training}
% For the generative dynamic model, 
% we propose a generic \GDM which consists of a generator $G$ 
% and a discriminator $D$, 
% trained adversarially w.r.t. the extended conditional Wasserstein metric 
% between two probability measures $\Prob_\varpi,\Prob_G$ 
% under a third probability measure $\Prob$;
% \begin{align}\label{eq:wasser}
% W(\Prob_\varpi,\Prob_G;\Prob):=&\sup\!_{D\in \|\cdot\|_L}\E_{\varpi\sim \Prob_\varpi|\varrho, \varrho\sim \Prob}[D(\varpi|\varrho)]-\E_{\varpi: G(\varrho\sim \Prob,z\sim\N(0,I))}[D(\varpi|\varrho)]
% \end{align}
% Here, $z$ is a mean-zero unit-variance Gaussian random vector
% and $\|\cdot\|_L$ indicates the space of $1$-Lipschitz functions. 
% In \GDM, $D$ solves the interior $\sup$, 
% while $G$'s objective is to minimize this distance 
% and learn the $\Prob_\varpi|\varrho$ for all $\varrho$. 
% In \GATS, $\Prob$ 
% is the distribution over pairs of $\varrho:(x,a)$ in the replay buffer, 
% and $\Prob_\varpi|\varrho$ is the distribution 
% over the successor states $\varpi:x'$, 
% as the transition kernel $T(x'|x,a)$.
